Towards a Unified View of Affinity-Based Knowledge Distillation

Knowledge transfer between artificial neural networks has become an important topic in deep learning. Among the open questions are what kind of knowledge needs to be preserved for the transfer, and how it can be effectively achieved. Several recent work have shown good performance of distillation methods using relation-based knowledge. These algorithms are extremely attractive in that they are based on simple inter-sample similarities. Nevertheless, a proper metric of affinity and use of it in this context is far from well understood. In this paper, by explicitly modularising knowledge distillation into a framework of three components, i.e. affinity, normalisation, and loss, we give a unified treatment of these algorithms as well as study a number of unexplored combinations of the modules. With this framework we perform extensive evaluations of numerous distillation objectives for image classification, and obtain a few useful insights for effective design choices while demonstrating how relation-based knowledge distillation could achieve comparable performance to the state of the art in spite of the simplicity.

==> figures/banner.tex <==
\usetikzlibrary{arrows,shapes.geometric,positioning}%
\begin{tikzpicture}[align=center, node distance = 1mm]%
\node[align=center] (fl) {Loss};%
\node[above left= 1mm and -2mm of fl] (fn1) {Normalization};%
\node[above= of fn1] (fa1) {Affinity};%
\node[above= of fa1] (st) {Student};%
\node[above right= 1mm and -2mm of fl] (fn2) {Normalization};%
\node[above= of fn2] (fa2) {Affinity};%
\node[above= of fa2] (Te) {Teacher};%
\end{tikzpicture}%

==> figures/tables/TL_experiments.tex <==
\begin{tabular}{llllll}
\toprule
         &     & baseline &          kd & mAKD init\_beta=8.0 & mAKD init\_beta=0.0 \\
\midrule
resnet18 & Dogs &    76.71 &  79.73$\pm$0.22 &         79.10$\pm$0.33 &         78.77$\pm$0.14 \\
         & Flowers &    93.38 &  95.53$\pm$0.16 &         94.81$\pm$0.11 &         93.50$\pm$0.14 \\
         & CUB &    73.84 &  77.00$\pm$0.29 &         75.50$\pm$0.27 &         72.77$\pm$0.37 \\
resnet34 & Dogs &    80.90 &  82.86$\pm$0.07 &         82.72$\pm$0.15 &         82.53$\pm$0.14 \\
         & Flowers &    94.54 &  96.10$\pm$0.17 &         95.63$\pm$0.07 &         94.68$\pm$0.28 \\
         & CUB &    76.35 &  79.54$\pm$0.16 &         78.66$\pm$0.18 &         76.38$\pm$0.17 \\
\bottomrule
\end{tabular}


==> figures/tables/comparison-v2-wo_sd.tex <==
\begin{tabular}{llllllll}
    \toprule
               &              & \multicolumn{3}{l}{top1} & \multicolumn{3}{l}{top5}                                                                                     \\
            Teacher(T)   & Student(S)             & T/S          & CRD                      & mAKD           & T/S & CRD                 & mAKD           \\
    \midrule
    ResNet50   & MobileNetV2  & 78.68/64.34              & \textbf{69.21}      & 68.87          & 95.32/87.67     & 90.87          & \textbf{91.49} \\
               & vgg8         & 78.68/70.28              & 74.02               & \textbf{74.37} & 95.32/90.29     & 92.86          & \textbf{93.37} \\
    ResNet110  & ResNet20     & 73.90/69.30              & \textbf{71.24}      & 70.39          & 92.92/91.89     & \textbf{92.51} & 92.42          \\
               & ResNet32     & 73.90/71.00              & \textbf{73.27}      & 72.88          & 92.92/92.53     & 93.03          & \textbf{93.25} \\
    ResNet32x4 & ShuffleNetV1 & 79.06/71.55              & 75.28               & \textbf{75.59} & 94.64/91.20     & 93.29          & \textbf{93.86} \\
               & ShuffleNetV2 & 79.06/72.42              & 75.77               & \textbf{75.97} & 94.64/91.67     & 93.73          & \textbf{94.02} \\
               & ResNet8x4    & 79.06/72.54              & \textbf{75.37}      & 74.60          & 94.64/92.44     & \textbf{94.02} & 93.96          \\
    ResNet56   & ResNet20     & 72.72/69.30              & \textbf{71.18}      & 70.32          & 92.35/91.89     & 92.46          & \textbf{92.73} \\
    vgg13      & MobileNetV2  & 74.88/64.34              & \textbf{69.07}      & 68.12          & 92.73/87.67     & \textbf{91.22} & 90.99          \\
               & vgg8         & 74.88/70.28              & 73.42              & \textbf{73.73} & 92.73/90.29     & 92.67          & \textbf{92.72} \\
    WRN-40-2   & ShuffleNetV1 & 76.17/71.55              & 75.68               & \textbf{76.15} & 93.55/91.20     & 93.40          & \textbf{94.07} \\
               & WRN-16-2     & 76.17/73.44              & \textbf{75.53}      & 75.30          & 93.55/93.05     & 93.99          & \textbf{94.21} \\
               & WRN-40-1     & 76.17/71.39              & \textbf{74.09}      & 73.78          & 93.55/92.40     & 92.93          & \textbf{93.54} \\
    \bottomrule
\end{tabular}


==> figures/tables/comparison.tex <==
\begin{tabular}{lllllllll}
\toprule
         &              & \multicolumn{3}{l}{CRD results [Acc]} & \multicolumn{4}{l}{Our results [Acc]} \\
         &              & Teacher / Student &     KD &    CRD & Teacher / Student &   CS L2 KL 2.0 &   CS L2 KL 2.5 &  CS L2 SL1 1.0 \\
Teacher & Student &                   &        &        &                   &                &                &                \\
\midrule
wrn-40-2 & wrn-16-2 &     75.61 / 73.26 &  74.92 &  75.48 &     76.37 / 72.48 &  75.17 +- 0.18 &  75.45 +- 0.21 &  75.01 +- 0.24 \\
         & wrn-40-1 &     75.61 / 71.98 &  73.54 &  74.14 &     76.37 / 71.73 &  73.61 +- 0.30 &  74.01 +- 0.33 &  73.65 +- 0.21 \\
resnet56 & resnet20 &     72.34 / 69.06 &  70.66 &  71.16 &     72.35 / 69.00 &  70.58 +- 0.15 &  70.56 +- 0.21 &  70.89 +- 0.12 \\
resnet110 & resnet20 &     74.31 / 69.06 &  70.67 &  71.46 &     74.56 / 69.00 &  71.00 +- 0.11 &  70.41 +- 0.26 &  70.91 +- 0.18 \\
         & resnet32 &     74.31 / 71.14 &  73.08 &  73.48 &     74.56 / 71.26 &  73.10 +- 0.25 &  73.09 +- 0.24 &  72.88 +- 0.49 \\
resnet32x4 & resnet8x4 &     79.42 / 72.50 &  73.33 &  75.51 &     79.20 / 72.32 &  74.44 +- 0.37 &  74.33 +- 0.09 &  74.38 +- 0.04 \\
vgg13 & vgg8 &     74.64 / 70.36 &  72.98 &  73.94 &     74.55 / 70.55 &  73.69 +- 0.17 &  73.86 +- 0.19 &   73.70 +- nan \\
         & MobileNetV2 &     74.64 / 64.60 &  67.37 &  69.73 &     74.55 / 64.16 &  68.69 +- 0.19 &  68.27 +- 0.72 &  68.22 +- 1.00 \\
ResNet50 & MobileNetV2 &     79.34 / 64.60 &  67.35 &  69.11 &     78.46 / 64.16 &  68.84 +- 0.67 &  68.60 +- 0.68 &  68.73 +- 0.59 \\
         & vgg8 &     79.34 / 70.36 &  73.81 &  74.30 &     78.46 / 70.55 &  73.93 +- 0.16 &  74.07 +- 0.31 &  73.65 +- 0.37 \\
resnet32x4 & ShuffleNetV1 &     79.42 / 70.50 &  74.07 &  75.11 &     79.20 / 72.15 &  74.22 +- 0.36 &  74.28 +- 0.31 &  74.16 +- 0.24 \\
         & ShuffleNetV2 &     79.42 / 71.82 &  74.45 &  75.65 &     79.20 / 72.14 &  75.51 +- 0.38 &  75.56 +- 0.21 &  75.45 +- 0.18 \\
wrn-40-2 & ShuffleNetV1 &     75.61 / 70.50 &  74.83 &  76.05 &     76.37 / 72.15 &  75.64 +- 0.20 &  75.30 +- 0.40 &  74.89 +- 0.20 \\
\bottomrule
\end{tabular}


==> figures/tables/imnet_comparison.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
{} &  Teacher &  Student &    AT &     KD &     SP &     CC &    CRD &  CRD+KD \\
\midrule
Top-1 &    26.69 &    30.25 &  29.3 &  29.34 &  29.38 &  30.04 &  28.83 &   28.62 \\
Top-5 &     8.58 &    10.93 &  10.0 &  10.12 &  10.20 &  10.83 &   9.87 &    9.51 \\
\bottomrule
\end{tabular}


==> figures/tables/self-kd.tex <==
\begin{tabular}{lllll}
\toprule
{} & Baseline &   Self mAKD & Relative difference & Absolute difference \\
\midrule
resnet8      &    60.40 &  58.44$\pm$0.23 &              -3.25\% &               -1.96 \\
resnet14     &    68.01 &  67.49$\pm$0.12 &              -0.76\% &               -0.52 \\
wrn-16-1     &    67.07 &  66.77$\pm$0.19 &              -0.44\% &               -0.30 \\
resnet8x4    &    72.54 &  72.34$\pm$0.26 &              -0.28\% &               -0.20 \\
resnet20     &    69.30 &  69.19$\pm$0.13 &              -0.16\% &               -0.11 \\
wrn-16-2     &    73.44 &  73.80$\pm$0.30 &               0.48\% &                0.36 \\
vgg8         &    70.28 &  70.82$\pm$0.19 &               0.77\% &                0.54 \\
resnet32x4   &    79.06 &  79.79$\pm$0.23 &               0.93\% &                0.73 \\
vgg19        &    73.70 &  74.51$\pm$0.16 &               1.09\% &                0.81 \\
ResNet50     &    78.68 &  79.63$\pm$0.14 &               1.20\% &                0.95 \\
vgg16        &    74.59 &  75.51$\pm$0.33 &               1.23\% &                0.92 \\
vgg13        &    74.88 &  76.02$\pm$0.22 &               1.52\% &                1.14 \\
resnet44     &    72.64 &  73.76$\pm$0.21 &               1.55\% &                1.12 \\
resnet56     &    72.72 &  74.03$\pm$0.19 &               1.81\% &                1.31 \\
wrn-40-2     &    76.17 &  77.61$\pm$0.13 &               1.89\% &                1.44 \\
vgg11        &    71.72 &  73.08$\pm$0.15 &               1.90\% &                1.36 \\
resnet32     &    71.00 &  72.38$\pm$0.37 &               1.94\% &                1.38 \\
ShuffleNetV1 &    71.55 &  72.96$\pm$0.26 &               1.97\% &                1.41 \\
resnet110    &    73.90 &  75.57$\pm$0.25 &               2.27\% &                1.67 \\
wrn-40-1     &    71.39 &  73.40$\pm$0.20 &               2.81\% &                2.01 \\
ShuffleNetV2 &    72.42 &  74.56$\pm$0.12 &               2.95\% &                2.14 \\
MobileNetV2  &    64.34 &  67.20$\pm$0.27 &               4.45\% &                2.86 \\
\bottomrule
\end{tabular}


==> sections/discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\textbf{Inner product based metric is a better affinity:} % metric than distance:}
Based on the observations from our experiments we can deduce that the choice of the affinity module is a dominating factor in constructing a good mAKD objective. In our setup for image classification where we applied mAKD to the penultimate layer, we saw a considerable benefit in using inner product based affinity functions, i.e. $\tt{CS}$ and $\tt{IP}$, as opposed to $\tt{L1}/\tt{L2}$. Our conjecture is that the advantage is derived from a better alignment between the inner product based affinity module and the operations performed in the classification layer. 
Namely, while the classification layer computes the inner product of the sample and class representation, those affinity modules also compute the inner product of the sample representations within a batch.
This analogy holds in our setup although other insights could be obtained in different applications of mAKD.
%That is, row $i$ of the weight matrix in that layer corresponds to the prototype vector learned for class $i$. 
%The inner product of the feature vector and the prototype vector defines the affinity between the sample and the class representation. 
% This operation can be seen as corresponding to the inner product based affinity with the difference that the 
% while inner sample and class distribution
%On the other hand, the purpose of the affinity module is to compute the similarity/dissimilarity between the sample representations within a batch, where the process based on the inner product is essentially equivalent to the propagation through the classification layer. 

\textbf{Normalisation is important but less so for cosine similarity:}
% Multiple observations are made for the normalisation of the affinity matrix. 
For the normalisation of the affinity matrix
the most notable among available observations can be explained as: % follows: 
$a.$ we should use normalisation, $b.$ we should avoid max normalisation, and $c.$ the choice of normalisation is less important for cosine similarity affinity module. 

$a.$ When distilling knowledge from teacher to student % the aim is to pick a student model 
that is more compact, the compactness of the student model implies that it has lower capacity than the teacher. Therefore it is usually hard for a student model to exactly mimic the manifold of teacher's representation. By applying normalisation 
% we are able to weaken such constraint. 
such a restriction is expected to be softened.

$b.$ All the normalisation functions do not work equally; row-wise normalisation and normalisation by the  average value achieve better performance than the one based on the maximum value. We believe that this is due to imbalance in the affinity scores among different pairs. That is, a certain pair of samples may well result in an affinity value that is much greater than the rest. Such a value used as the max normalisation factor will cause loss of information since most of the normalised values will become negligibly small.

$c.$ $\tt{CS}$ achieves good performance across a diverse set of normalisation functions including max normalisation. This is explained by virtue of internal normalisation of the cosine similarity metric.

\textbf{The choice of loss function is less important:}
When we pick row-wise normalisation or normalisation by average, the choice of loss function has smaller impact on the performance of the mAKD objective. To be noted is that KL divergence benefits from any normalisation. This is likely thanks to a similar effect to that by the temperature scaling in original Knowledge Distillation \cite{hinton2015distilling}, where normalisation factor (inverse temperature) smaller than one has a smoothing effect on softmax distribution, which helps recover the hidden affinity between sample pairs. 
% To be noted is that KL divergence benefits from any normalisation, and this is likely thanks to a similar effect from the temperature scaling with its normalisation factor (temperature) greater than one, which smooths out the softmax distribution.


\textbf{Benefits of GNoRP:} There are two benefits in using GNoRP instead of static weighting: $a.$ it {\it absorbs} the differences that occur due to different architectures or different definitions of the loss functions and $b.$ it allows for better interpretability of the GradNorm ratio $r_{GN}$, 
%as opposed to 
than
the weighting parameter $\lambda$. Both benefits are related to the fact that controlling GradNorm ratio has a more direct effect on the update of models parameters than a static weighting of the losses. Since the gradient norm is approximately proportional to the step made in the parameter space, the GradNorm ratio $r_{GN}$ would correspond to the ratio of step sizes from the two losses. For example, setting $r_{GN} = 2$ implies that the step size due to the mAKD loss is twice as large as that due to the main loss. Following this explanation we can interpret the gradient norm ratio as the importance ratio between the losses. Furthermore, if a hyper-parameter search is too expensive, one could use an uninformative prior $r_{GN}=1$, signifying that the two losses are given an equal importance. 
%Furthermore, note how different definition of the loss functions, e.g. whether we sum or average across the batch, and different dimensionality of the feature vector across different architectures results in diversity of loss value. One could expect that using same weighting value across such diversity is impractical.  Therefore using same value for weighting is often impractical 


% \textbf{Interpretability of GradNorm ratio preservation:}
% The size of the step during the parameter optimisation is in proportional relation to the magnitude of gradient. A good balance is important for good convergence; a too small step size will slow down the convergence whereare a large step will make it unstable. As such, balancing the gradient norm is more directly connected than weighting of loss functions to the manipulation of the gradient magnitude. By ensuring that the ratio of gradient norms between the two losses has a fixed value $r_{GN}$, as we do in GNoRP, we can interpret this such that the ratio of the gradient magnitude is maintained (?) to $r_{GN}$. Hence, applying a ratio, $r_{GN}=2$, to our setup is equivalent to claim that the gradient from mAKD loss is twice as large as the counterpart from the classification loss. If a hyper-parameter search is to expensive, one could use an uninformative prior $r_{GN}=1$, signifying that the two losses are equally important. 

\textbf{Advantage in the top-5 accuracy:}
the mAKD loss tends to give better performance in terms of top-5 accuracy, in particular, with mAKD($\tt{CS}$ $\tt{L2}$ $\tt{KL}$) as seen in section \ref{sec:comarison_with_sota}. 
Our intuitive interpretation is that mAKD can be better suited to capture the class similarity intrinsic to given training data, e.g. {\it cat} is a closer category to that of {\it dog} than {\it bus}.
This could bring further benefit in open set classification problem settings where a sample that does not have a clear association to one single class, but it could be explained as a combination of multiple categories.
% Potential benefit of such knowledge can be seen when we analyse a sample that does not have a clear association to one single class.

% Potential advantage of awareness of the class similarity can be explained in following example: assume that we have a model that is trained on three classes; 
% Our intuitive explanation is that relation-based knowledge is more suited than instance-based one to capture the class similarities intrinsic to given training data.
% , as a method for capturing relation-based knowledge, 
% than CRD 
%in addition to capturing the inter-class similarity, 
% That is, mAKD objective more rigorously captures the knowledge about relation between the classes .

















\textbf{Applications of mAKD framework:}
We have investigated a variety of affinity based objectives in the mAKD framework, thus far on image classification tasks. If one would like to use mAKD framework in a similar setup we strongly recommend to use one of the best performing variants shown in figure \ref{fig:initial_exp_color}. When using mAKD in a different setup, however, our recommendation is to construct a combinatorial search. We believe that without loss of generality one can reduce the search space to the following modules: $\tt{CS}$ and $\tt{L2}$ for affinity metric, $\tt{L2}$ normalisation, and $\tt{KL}$ and $\tt{SL1}$ as  loss functions. However, the mAKD framework is not restricted to the modules presented in this paper, therefore we would like to encourage extensions of mAKD with other modules that might be better suited to the task at hand.

% In this section we will try to give an intuitive explanation to why the inner product based affinity metrics is a better choice for mAKD loss. If we disregard the bias term in the linear classification layer, we are left with an inner product between the classifier weights $W_{cls}$ and the penultimate features. If we consider each row of $W_{cls}$ being the "prototype" feature for each class, then the linear classifier would represent the IP affinity between the class prototype and the feature vector. If the IP affinity between sample $i$ and prototype $j$ is higher then the rest of the prototypes we assign class $j$ to that sample. In case of mAKD loss, instead of computing affinity between the feature and a prototype vector, we use the features from other samples instead of the learned prototype vectors. Using this analogy we would like to argue that inner product based affinity is better aligned to the classification operation of the last layer, and therefore allow for better performance then the distance based metrics. 

% The first observation can be explained by the fact that inner product based affinity has better alignment with the operations performed in the last classification layer (see section \ref{sec:discussion}). Furthermore the CS affinity performs the same operation as IP affinity with an addition of normalisation of the feature vectors.  

% While row wise normalisation in general works well we notice that max normalisation has worst performance. Using max normalisation is unstable because there might be a large difference between the maximum of an affinity matrix and the rest of the values. When normalised with maximum of the affinity matrix, a lot of information is lost, as most of the values becomes negligibly small. Note that max normalisation is not affecting the performance when used with KL divergence. That is explained by the fact that softmax is used before the KL divergence. Furthermore, since the max value of CS affinity is 1, max normalisation has no effect when used in the combination with CS affinity.

% Due to inherit normalisation in the CS affinity and softmax normalisation in the KL loss, the performance is good for any normalisation function for the CS affinity paired with KL loss.

% Inpretability of alpha
% We would like to argue that the effect of the gradient norm is more direct then the weighting of the loss function. Therefore by using  GradNorm ratio preservation, as opposed to setting a static weighting parameter $\lambda$, we gain better interpretability. For example if the ratio $r_{GN}$ is set to two, then we can interpret that as the importance for the secondary loss is two times higher than the importance of the main loss. However, the same cannot be said about the magnitude ratio between the loss functions.

% TODO: discus why top 5 accuracy can be beneficial. 

==> sections/introduction.tex <==
\section{Introduction}%
\label{sec:Introduction}%
It has been demonstrated that deeper and wider deep neural networks (DNN) often have benefits  in their performance over the smaller counterparts \cite{he2016deep, zagoruyko2016wide}. The size of DNNs can however be an issue  in their deployment for production; due to a large memory footprint or substantial computational cost, those models may not necessarily fit well to small devices with limited power capacity, e.g.  a mobile phone.
%
While different approaches have been proposed to cope with this problem, such as designing effective architectures \cite{howard2017mobilenets, zhang2018shufflenet}, model pruning \cite{han2015learning, molchanov2016pruning}, low-rank approximation \cite{denton2014exploiting, jaderberg2014speeding}, and model quantization \cite{bulat2017binarized, lin2016fixed}, research based on knowledge transfer have shown promising directions in terms of knowledge distillation (KD), or distillation in short, which this paper is also concerned with. 

\begin{figure}
    \centering
    \includegraphics[width=0.39\textwidth,trim=25 13 9 15, clip]{figures/banner3.pdf}
    \caption{A schematic of the proposed framework, modular Affinity-based Knowledge Distillation (mAKD), defining a new objective $L_{\text{mAKD}}$. It consists of three components; affinity, normalisation, and loss. Each component has modules, described in section \ref{subsec:CombinatorialRelationalKnowledgeDistillation}, that can be swapped independently. 
    %The affinity is computed for every pair of samples in the batch.
    }
    \label{fig:banner}
\end{figure}

The basic idea of knowledge transfer is to encode useful knowledge of  data by a bulky teacher model and use that for training a smaller student network. Buciluǎ et al. \cite{bucilua2006model} were among the first that introduced knowledge transfer  in the context of artificial neural networks. They used a large ensemble to label training data, and the labelled data were used to train a single neural network. Similar ideas were utilised in \cite{hinton2015distilling, ba2014deep, zagoruyko2016paying, ahn2019variational, romero2014fitnets} where a cumbersome model was used to assist training of a smaller, shallower network. It should be noted that all these methods
% To be noted is that those all 
use individual knowledge from single sample encoding/embedding which is referred to as instance-based knowledge.

More recent work looked at distillation using relation-based knowledge, i.e. relationships among representations of samples \cite{tung2019similarity, park2019relational, passalis2018learning, peng2019correlation}. Those compelling methods share a common aim of capturing the relations among embeddings as intra-batch knowledge and contributed to improvements in performance. Yet, there is a considerable variation between them, e.g. in terms of affinity measures, and valid comparisons are missing. Hence, it is a challenging open question to motivate possible definitions of the relationship for the purpose of effective distillation. 
% How to effectively extract relation-based knowledge?
% also due to the lack of valid comparisons between the existing methods.

The primary goal of this paper is to explore this question by a systematic study of putting possible variations in a modular framework covering most of the existing relation-based knowledge distillation and other more. Such a framework allows us to perform a rigorous comparison between different variants in a controlled setting. We call our framework a modular Affinity-based Knowledge Distillation (mAKD) which is composed of three components, see figure \ref{fig:banner}. Each component's modules can independently be swapped, resulting in numerous possible combinations (we consider 80 of them in our experiments). Using mAKD, we conduct a set of empirical experiments to identify well performing combinations (as well as certain variants to avoid) while providing some insights explaining them.


Our auxiliary goal is to find a good balance between the main objective, i.e. cross-entropy loss for image classification in our case, and the Knowledge Distillation objective.
% Our auxiliary goal is to find a good balance between the Knowledge Distillation and the main objectives. In our case the main objective is cross-entropy loss for image classification.
%It is a common practice to combine the distillation loss with the main target loss, i.e. cross-entropy loss for a classification problem, using a certain weight. 
Although the interplay between the two is generally complex and not well understood, here we employ a strategy that we call GradNorm ratio preservation (GNoRP) which is inspired by the GradNorm \cite{chen2018gradnorm}. The aim of the GradNorm in the case of multitask learning setting is to balance the losses so that the training rate for each task is kept equivalent; the balancing is achieved by adjusting weighting factors, one for each task loss, such that the discrepancy between the gradient norms gets decreased. Unlike the GradNorm we only use a single weighting parameter $\lambda$ which we dynamically adjust in such a way that the ratio between the gradient norms of the two losses remains constant. Such adaptation of GradNorm simplifies the method and allows for an interpretability of the GradNorm ratio (see section \ref{sec:discussion}).

In sum, our contributions are:
\begin{itemize}
    \item
          A family of modular distillation functions, called modular Affinity-based Knowledge Distillation (mAKD).

    \item
          An extensive comparison between mAKD variants, leading to guidelines for effective design choices.
          
    \item
          A method for dynamically adjusting weighting of the additional loss, termed GradNorm ratio preservation (GNoRP).
\end{itemize}
%In addition to the three contributions listed above, we also demonstrate that mAKD is able to achieve at least equivalent performance to this state-of-the-art method.
% of Knowledge Distillation \cite{tian2019contrastive}. 
The authors of \cite{tian2019contrastive} have proposed contrastive representation distillation (CRD) and performed a comprehensive comparison with multiple distillation losses on a large variety of teacher student pairs, and demonstrated the state-of-the-art performance. 
In addition to the three contributions listed above, we also show that mAKD is able to achieve equivalent performance to this state of the art.%, and outperform the teacher network more often.
% For a fair comparison with CRD, we also employ a common set of architectures and hyper-parameters that were made publicly available by the authors of \cite{tian2019contrastive}.


==> sections/method.tex <==
\label{sec:Method}%
\section{Method}%
This section is divided into three parts, each part corresponding to one of the contributions listed in section \ref{sec:Introduction}. First we describe components and modules that constitute the mAKD framework (section \ref{subsec:CombinatorialRelationalKnowledgeDistillation}), followed by the description of the combinatorial search (section \ref{subsec:Combinatorialsearch}) and GradNorm ratio preservation (section \ref{subsec:Dynamicbeta}). 

\subsection{Modular Affinity-based Knowledge Distillation}%
\label{subsec:CombinatorialRelationalKnowledgeDistillation}%
Given two ANN models, a pre-trained teacher $f^{(T)}$ and a randomly initialised student $f^{(S)}$, the goal of Knowledge Distillation is to train the student model with an assistance of the teacher model. A standard way to perform Knowledge Distillation is to define an additional loss function that is based on teacher's and student's representations. The main loss and a weighted KD loss are then jointly optimised using the loss function:%
\begin{equation}%
      L = L_{\text{main}} + \lambda \sum_{(l,l')} L_{\text{KD}}(z^{(S,l)}, z^{(T,l')})%
      \label{eq:weightedLoss}%
\end{equation}%
where $z^{(S,l)}$ and $z^{(T,l')}$ are feature representations of a batch produced by layer $l$ of the student and layer $l'$ of the teacher network, respectively. For simplicity, 
% we choose feature representations to be the output of the penultimate layers. 
we consider the output of the penultimate layers as the feature representations. 
Without loss of generality, however, our method can be extended to any layers in the teacher-student pair.%

The modular Affinity-based Knowledge Distillation (mAKD) objective consists of three main components: affinity metric $g$, normalisation of affinity matrix $f$, and a loss function $L$. $g$ is a measure of similarity/dissimilarity between samples within a batch. $f$ is used to relax the constraint of the mAKD objective in terms of the absolute magnitude of the affinity. 
% $L$ is to minimise the discrepancy between the normalised affinity matrices both from the student and teacher networks. 
$L$ defines the loss to minimise the discrepancy between the normalised affinity matrices from the student and teacher networks. 
Given the batch of penultimate feature representations from teacher $z^T$ and student $z^S$, the total loss is defined as:
\begin{equation}%
      L = L_{\text{main}} + \lambda L_{\text{mAKD}}(z^S, z^T)%
      \label{eq:totalLossFunc}%
%      \vspace{-3mm}%
\end{equation}%
where $L_{\text{mAKD}}$ is the mAKD objective:
\begin{equation}
    L_{\text{mAKD}}(z^S, z^T) = L(f(g(z^S)), f(g(z^T)))
    \label{eq:makd_objective}
\end{equation}
The concept in equation \ref{eq:makd_objective} is depicted in figure \ref{fig:banner}.

\subsubsection{Affinity metric}%
\label{ssubsec:Affinitymetric}%
Different pairwise affinity metrics have been proposed in the literature. For this study we choose affinity metrics according to two conditions: $a.$ simplicity of the metric and $b.$ the metric does not introduce additional parameters. The affinity function $g$ assigns a similarity score for every pair of samples in the batch. It creates an affinity matrix $G$ whose element $G_{i,j}$ corresponds to the affinity score between sample $i$ and sample $j$, $G_{i,j} = g(z_i, z_j)$. Note that affinity matrix $G$ is computed independently for teacher and student.%

\textbf{Norm based affinity:} The simplest measures of affinity are the Manhattan and Euclidean distance, referred to as L1 and L2, respectively. Given two feature vectors $z_i$ and $z_j$, the two metrics are:%
\begin{alignat}{2}%
      g_{\tt{L1}}(z_{i}, z_{j}) & = \norm{z_{i}-z_{j}}_1 \\%
      g_{\tt{L2}}(z_{i}, z_{j}) & = \norm{z_{i}-z_{j}}_2 %
\end{alignat}%

\textbf{Inner product based affinity:} Another way to measure the affinity is by the inner product between the two vectors. We consider the Inner Product ($\tt{IP}$) and Cosine Similarity ($\tt{CS}$) as candidates for the affinity metric.%
\begin{alignat}{2}%
      g_{\tt{IP}}(z_{i}, z_{j}) & = \sum_k z_{i,k}z_{j,k}                                          \\%
      g_{\tt{CS}}(z_{i}, z_{j}) & = \frac{\sum_k z_{i,k}z_{j,k}}{\norm{z_{i}}_2\norm{z_{j}}_2} %
\end{alignat}%
In total those make four affinity metrics: L1/L2 distances ($\tt{L1}/\tt{L2}$) and Inner Product ($\tt{IP}$), and Cosine Similarity ($\tt{CS}$).

\subsubsection{Normalisation}%
\label{ssubsec:Normalisation}%
Given the affinity matrix $G$, a normalisation can be performed in multiple ways. Let function $f$ represent a normalisation function, and the normalised affinity matrix $\tilde{G} = f(G)$.

\textbf{Row-wise normalisation:} We can consider each row of $G$ as the affinity vector, $G_i$. $G_i$ conveys information about the similarity/dissimilarity of sample $i$ to all samples in the batch. Row-wise normalisation ensures that each affinity vector has a unit L1- or L2-norm.%
\begin{alignat}{2}%
      f_{\tt{L1}}(G) = \frac{G_{i,j}}{\norm{G_{i,:}}_1} \\%
      f_{\tt{L2}}(G) = \frac{G_{i,j}}{\norm{G_{i,:}}_2}%
\end{alignat}%

\textbf{Matrix normalisation:} We can use the statistics of the entire affinity matrix, and consider average- and max-normalisation. In the former, the average across all elements in $G$ is made equal to one unit, whereas in the latter, the maximum value in $G$ is made equal to one unit.%
\begin{alignat}{2}%
      f_{\tt{avg}}(G) & = \frac{b^2}{\sum_{i,j} G_{i,j}}G_{i,j} \\%
      f_{\tt{max}}(G)  & = \frac{G_{i,j}}{\max(G_{i,j})}          %
\end{alignat}%
where $b$ is the batch size.

\textbf{No normalisation ($\tt{noN}$):} If important information is hidden in the magnitude of the affinity metric we want to keep that information. Hence, not applying normalisation is a reasonable option.

In total we investigate five alternatives, i.e. L1/L2 row-wise normalisation ($\tt{L1}/\tt{L2}$), average/maximum ($\tt{avg}/\tt{max}$) matrix normalisation, and No normalisation ($\tt{noN}$).

\subsubsection{Loss function}%
\label{ssubsec:Lossfunction}%
The remaining component of mAKD is to compare the normalised affinity matrices from student and teacher networks. We define a loss such that the student learns to mimic inter-sample relations encoded by the affinity and normalisation functions. We investigate four different loss functions: three regression losses and KL divergence.

\textbf{Regression losses:} The aim of the regression losses is to reduce the discrepancy between the normalised affinity matrices. We use L1/L2 distance, and a combination of both, i.e. SmoothL1 ($\tt{SL1}$) loss.%

\begin{equation}
      L(\tilde{G}^{(S)}, \tilde{G}^{(T)}) = 
    %   \frac{1}{b^2}
      \sum_{i,j} L_{\text{reg}}(\tilde{G}_{i,j}^{(S)}-\tilde{G}_{i,j}^{(T)})
\end{equation}
where $L_{\text{reg}}$ is defined for given input $x$ as:
\begin{alignat}{3}
      L_{\tt{L1}}(x)       & = \left|x\right|            \\
      L_{\tt{L2}}(x)       & = x^2                       \\
      L_{\tt{SL1}}(x) & = \begin{cases}
            0.5x^2 & \text{if } x < 1.0 \\
            x-0.5  & \text{otherwise}
      \end{cases}
\end{alignat}

\textbf{KL divergence:} The most common divergence measure for probability distributions is KL divergence. To convert the affinity vectors into discrete probability distributions we use row-wise softmax before passing $\tilde{G}$ to KL divergence.%

\begin{alignat}{2}%
      L_{\tt{KL}}(\hat{G}^{(S)}, \hat{G}^{(T)}) & = %
      \dfrac{1}{b}
      \sum_{i,j} \hat{G}_{i,j}^{(T)}\log \dfrac{\hat{G}_{i,j}^{(T)}}{\hat{G}_{i,j}^{(S)}}
\end{alignat}%
where $\hat{G}_i = \text{softmax}(\tilde{G}_i)$.

In total we study four loss functions, i.e. L1/L2 distance ($\tt{L1}/\tt{L2}$), SmoothL1 loss ($\tt{SL1}$), and KL divergence ($\tt{KL}$). 

\subsubsection{mAKD loss and its connection to the related work}
The mAKD objective is constructed by putting the modules, as described in the previous sections, into the three components.  We expect the chosen variations (80 combinations) to well cover important combinations although there can be other possible modules to be included. 
% certain variants that are not covered.
% it is nearly infeasible to investigate an exhaustive list in practice. 
Here, every mAKD variant is conveniently identified by an acronym triplet, corresponding to (affinity metric, normalisation method, loss function). For example, the objective function proposed in \cite{tung2019similarity} can be described as ($\tt{IP\ L2\ L2}$) while the distance-wise method in \cite{park2019relational} corresponds to ($\tt{L2\ avg\ SL1}$), and the bi-linear pooling version in \cite{peng2019correlation} to ($\tt{IP\ noN\ L2}$). In \cite{passalis2018learning} shifted and scaled Cosine Similarity is used, paired with L1 normalisation and KL divergence. Due to the nature of shifting and scaling Cosine Similarity, there is no corresponding mAKD variant, however it is closely related to ($\tt{CS\ L1\ KL}$).

As a convention we will use the acronym in the sequel for specific variants of mAKD, e.g. mAKD($\tt{CS\ L1\ KL}$).
%
\subsection{Combinatorial search}%
\label{subsec:Combinatorialsearch}%
To find the most effective and meaningful combinations, we designed a combinatorial search. For a proper comparison between different mAKD variants we imposed the following requirements:
\begin{enumerate}[i]
      \item The mAKD loss should be tested in isolation.%
      \item The effect of any mAKD variant, on the update of the model, should be equal to each other. 
    %   \item No extra parameters are added.%
\end{enumerate}%
To conform the first requirement, we decomposed the model into two parts, a feature extractor (the entire model except the last classification layer) and a classifier. A variant of mAKD loss was used to train a feature extractor. To validate the effectiveness of the loss, we trained a linear classifier with the features extracted from the training set. We use the validation accuracy of the classifier as the performance metric for all the mAKD variants.%

The second requirement is fulfilled by weighting mAKD objective by a fixed $\lambda$. 
$\lambda$ is chosen such that the initial gradient norm of the mAKD is made equal to the average value of the initial gradient norm ($0.07$ units) that is observed when different randomly initialised models are trained with classification loss only. Note that the gradient norm is w.r.t. the penultimate feature vector $z$.
% . to that of the classification loss which appears when training with cross-entropy only.  and only one of the mAKD variants is used at one time (?) in the combinatorial search. 
% w.r.t. the penultimate feature vector is equal to that w.r.t. the corresponding feature vector obtained during the normal training, i.e. training  with classification objective only. 
% The $\lambda$ is chosen such that the initial gradient norm w.r.t. the penultimate feature vector is equal to that w.r.t. the corresponding feature vector obtained during the normal training, i.e. training  with classification objective only. 
% The initial gradient norm is set to $0.07$ units, in accordance with our observations coming from different randomly initialised teacher-student architecture pairs.
By applying such $\lambda$, we are able to ensure that different mAKD variants have equal importance on the update of the model parameters, resulting in a better comparison. %

% The third requirement is satisfied by choosing 
Furthermore, we use the same set of hyper-parameters as used in the training with classification loss only. Doing so, it is safe to regard that 
additional 
% introduced 
distillation loss will have stable convergence when paired with the original loss.

\subsection{Gradient Norm Ratio Preservation (GNoRP)}%
\label{subsec:Dynamicbeta}%
It is natural to anticipate that the optimal weighting parameter $\lambda$ (see equation \ref{eq:totalLossFunc}) can be different for different mAKD variants as well as for different teacher-student architecture pairs. In fact, during our experiments we observed varying impacts on the update of the parameters for different mAKD objectives. This was also the case with an identical mAKD variant applied to different teacher-student pairs. 

To deal with this matter, we propose a method for dynamic adjustment of $\lambda$ which is inspired by the GradNorm \cite{chen2018gradnorm}. Unlike GradNorm, however, we relax the objective and simply adjust $\lambda$, with every new mini-batch, so that the gradient norm ratio, $r_{GN}$, between the main classification criterion and the mAKD objective is kept constant. We compute the gradient norm with respect to the penultimate feature representation $z$. $\lambda$ is obtained by an  optimisation of following loss function:

\begin{equation}
    L_{\text{GNoRP}} = 
    \left(
    r_{GN} \norm{\dfrac{\partial L_{\text{main}}}{\partial z}}_2 - \norm{\dfrac{\partial \lambda L_{\text{mAKD}}}{\partial z}}_2
    \right)^2
\end{equation}
where $L_{\text{main}}$ and $L_{\text{mAKD}}$ denote classification loss and mAKD loss, respectively. %, and $r_{GN}$ indicates the ratio between the gradient norm of the two losses. 

%Using this formulation, we are able to find a single $r_{GN}$ that works across multiple settings.

Using this formulation, we are able to examine different  values of $r_{GN}$ in order to find the one that works well across multiple settings.% while dynamically adjusting $\lambda$.

==> sections/related_work.tex <==
\section{Related work}
%There are mainly two categories of Knowledge Distillation (KD) methods, Instance-based KD (IKD) and Relational KD (RKD). IKD methods encodes "knowledge" using feature representation of single sample, while RKD methods aim to capture relational information (we term it affinity in this paper) between different samples' representation. 

%mAKD loss proposed in this paper is closely related to the losses in the RKD category introduced by \cite{park2019relational, passalis2018learning, peng2019correlation, tung2019similarity}. 
One of the most important factors in Knowledge Distillation is how to extract and transfer the knowledge. Mainly two types of knowledge have been considered:
% In knowledge distillation, the type of knowledge to be extracted (thence transferred) and the choice of teacher-student architectures for the transfer are two of the fundamental factors. With respect to the knowledge, mainly two types have been considered: 
$a.$ instance-based knowledge from individual samples, i.e. the outputs of a specific layer (whether logits or latent features), and $b.$ relation-based knowledge which involves relationships among representations of samples; 
we refer to the relationships as affinity in the sequel. Our focus in this paper is on how to exploit affinities, and the introduced mAKD is motivated by a few recent works \cite{park2019relational, passalis2018learning, peng2019correlation, tung2019similarity} that have explored this direction. 

In \cite{tung2019similarity}, the affinities between pairs of two sample representations were computed by their inner product, and stored in an affinity matrix for teacher and student network, respectively. Preceded by row-wise L2 normalisation, the mean squared error (MSE) was computed as the loss function between the teacher's and student's affinity matrices. 
%
In \cite{park2019relational}, the authors introduced two kinds of affinity metrics, distance-wise and angle-wise. The former is the Euclidean distance between every pair in the batch, normalised by the average of all the pairs, while the latter is to compute the cosine angle among every triplet in the batch. 
%The distance-wise metric is normalised by the average distance of the pairs in the batch.
Huber loss was used as the function for measuring the discrepancy between the two affinity matrices.
%
The authors of \cite{passalis2018learning} used a shifted and scaled version of the cosine similarity metric. The shift and scale are such that the range is always constrained to $[0,1]$. They used row-wise L1 normalisation to ensure that each row becomes a valid conditional probability, and KL divergence as the loss function. 
%
In \cite{peng2019correlation}, the authors considered three ways of measuring affinity: naive MMD, bi-linear pool, and Gaussian RBF. The bi-linear pooling is equivalent to the inner product in \cite{tung2019similarity}. MSE is used as the loss function. 

Across those successful work commonly exploiting relation-based knowledge, there is still a lack of consensus on how to extract the affinity in the most effective fashion. 
%
In this respect, however, we have identified a reoccurring composition of the proposed losses; they can be commonly regarded as consisting of an affinity-, normalisation-, and loss function. 
%Therefore, our proposed mAKD loss has three corresponding components.
According to the three components, we design the modular Affinity-based Knowledge Distillation that allows for fair, systematic, and extensive comparisons. 
%, as will be detailed in section \ref{subsec:CombinatorialRelationalKnowledgeDistillation}.

==> sections/results.tex <==
\section{Experiments}
We perform four groups of experiments. The first is to find a well-performing set of mAKD variants by a combinatorial search (section \ref{subsec:combinatorialsearchresults}). 
We then proceed with finding a proper gradient norm ratio $r_{GN}$ (section \ref{sec:alphasearch}). 
The results are compared with mAKD loss to the state of the art, i.e. CRD loss, on CIFAR100 and ImageNet datasets (section \ref{sec:comarison_with_sota}). Finally, GNoRP is validated by comparing its performance against the case with the best performing $\lambda$ for each T-S pair (section \ref{sec:dynamicBetaAblation}).
Those are followed by discussions in section \ref{sec:discussion}.
% We present our results and observations in the following sections. Further discussions on those observations are provided in section \ref{sec:discussion}.

\subsection{Combinatorial search}
\label{subsec:combinatorialsearchresults}
To find out the most meaningful combination of the mAKD loss we run eight experiments\footnote{Eight T-S pairs, which are the subset of the pairs used in \cite{tian2019contrastive}, as shown in the legend of figure \ref{fig:initial_exp_full}.}, for each of the 80 mAKD variants.
%
In figure \ref{fig:initial_exp_full} we report the validation accuracy (vertical-axis) for each T-S pair (different colours) and mAKD variants (along horizontal-axis). On the top plot we report all 80 mAKD variants sorted by the average accuracy, while top 20 best variants were reported on the plot in the bottom. From figure \ref{fig:initial_exp_full} we see that the $\tt{CS}$ affinity is consistently better than the rest. It is followed by related $\tt{IP}$ affinity and other distance based metrics. 
\begin{figure*}[ht!]
    \centering
    \includegraphics[width=\linewidth, trim=5 1 5 2, clip]{figures/plots/initial_exp_v2_sort_by_average.pdf}
    \caption{
    Results from the combinatorial search on CIFAR100. 
    Top figure for all mAKD variants and 20 best variants in the bottom.
    In both figures the horizontal-axis is for mAKD variants used to train a student model (not all the variants are indicated due to space in the top figure). The performance (in terms of the validation accuracy on the vertical-axis) was evaluated by training a linear classifier based on the features extracted from the model.
    % Validation accuracy on vertical axis, different mAKD variants on horizontal axis.
    See section \ref{subsec:CombinatorialRelationalKnowledgeDistillation} for the label abbreviations.
    % The labels are in short forms: Cosine Similarity$\rightarrow\tt{CS}$, Inner Product$\rightarrow\tt{IP}$, SmoothL1$\rightarrow\tt{SL1}$, and No normalisation$\rightarrow\tt{noN}$.
    % Upper plot shows results using all 80 mAKD combinations, while in the bottom plot best 20 combinations are shown.
    }
     
    \label{fig:initial_exp_full}
\end{figure*}

In a more intuitive visualisation over mAKD variants, in figure \ref{fig:initial_exp_color}, each cell corresponds to the average of normalised validation accuracy across different T-S pairs. The normalisation is performed such that the maximum accuracy for a T-S pair becomes equal to 1. Our observations based on figure \ref{fig:initial_exp_color} can be summarised as: 
\begin{itemize}
    \item the $\tt{CS}$ affinity has good performance across a wide range of normalisation and loss pairs, closely followed by the $\tt{IP}$ affinity.
    \item $\tt{max}$ normalisation has generally worse performance than other normalisation functions.
    \item $\tt{max}$ normalisation has reasonable performance for the $\tt{CS}$ affinity.
    \item $\tt{KL}$ loss works well for the $\tt{CS}$ affinity, across any normalisation functions.
    \item No normalisation ($\tt{noN}$) paired with the $\tt{KL}$ loss is consistently worse than any other normalisation for all affinity metrics except for the $\tt{CS}$ affinity.
    %For affinity metrics, except for $\tt{CS}$, KL loss paired with no normalisation is consistently worse than other normalisation functions.
\end{itemize}
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth, trim=6 7 11 6, clip]{figures/plots/initial_exp_color.pdf}
    \caption{
    Summary of combinatorial search for the same experiments that are shown in figure \ref{fig:initial_exp_full}. 
    Each subplot corresponds to a specific affinity metric, each row to a normalisation function, and each column to a different loss function. 
    The value on each cell is the average of normalised validation accuracy.
    %Note that $\tt{max}$ and $\tt{noN}$ combined with $\tt{CS}$ results in equivalent performance. Max value for $\tt{CS}$ is always equal to one, therefore applying $\tt{max}$ normalisation with $\tt{CS}$ affinity is equivalent to applying $\tt{noN}$ normalisation. 
    }
    \label{fig:initial_exp_color}
\end{figure*}

Using the insight obtained from the observations above, in further experiments we choose to use Cosine Similarity, L2 normalisation and SmoothL1 loss, i.e. mAKD($\tt{CS\ L2\ SL1}$). However, we would like to point out that the performance across the best 11 mAKD variants in figure \ref{fig:initial_exp_full} is similar to each other and any of those variants would work as well as or possibly better than the single choice we made above.

\subsection{Optimal GradNorm ratio, $r_{GN}$}
\label{sec:alphasearch}
In this experiment we investigate the effect of different $r_{GN}$, on CIFAR100. For every T-S pair, we run experiments by varying $r_{GN}$ from $0.5$ to $7$ with increment of $0.5$. The results are shown in figure \ref{fig:alpha_search}. Due to the variation in the accuracy across different T-S pairs, we perform a normalisation; the accuracy for each T-S pair is divided by the average across all $r_{GN}$ values. We can observe that the validation accuracy is increased with increasing $r_{GN}$, signifying the importance of the mAKD loss. The training accuracy is decreased with increasing $r_{GN}$, indicating that using mAKD reducing overfitting. Based on our observation we choose to use $r_{GN}=3.5$ in CIFAR100 experiments.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth, trim=6 6 6 6, clip]{figures/plots/alpha_search_accuracy.pdf}
    \caption{
    Normalised accuracy (along vertical-axis) for a range of $r_{GN}$ (horizontal-axis) as well as for different model pairs. 
    The performance (in blue) improved according to $r_{GN}$ up to $r_{GN}=3.5$. For $r_{GN}>3.5$ the validation accuracy plateaus while the variance is increased. 
    The training accuracy (orange) is decreased with increased $r_{GN}$.
    }
    \label{fig:alpha_search}
\end{figure}

\subsection{Comparison with the state-of-the-art}
\label{sec:comarison_with_sota}
\textbf{CIFAR100:} For a fair comparison with the state-of-the-art we rerun the experiments performed with the CRD loss \cite{tian2019contrastive}. In doing so we make sure that the pretrained teacher and random seeds are the same for CRD and mAKD experiments. For every T-S pair and each objective we had five runs with different random seeds. Note that the set of random seeds is kept the same. The teacher model is also kept the same across different runs. Table \ref{tab:crd_comparison} shows top-1 and top-5 test accuracy for CRD and mAKD ($\tt{CS\ L2\ SL1}$) losses. The performance of mAKD is comparable with CRD; while CRD is superior in terms of top-1 accuracy, mAKD has better performance in terms of top-5 accuracy. mAKD loss has especially good performance when the student model is vgg8 or one of the ShuffleNet versions. We would also like to note that standard deviation is considerably higher when using MobileNetV2 as the student network, indicating that the mAKD loss is sensitive to a good initialisation of MobileNetV2. 


\begin{table*}
    \centering
    \input{figures/tables/comparison-v2.tex}
    \caption{Average test accuracy in using different T-S pairs (for CIFAR100) and its standard deviation across five independent runs with different seeds. For this comparison we use $r_{GN}=3.5$ and mAKD($\tt{CS\ L2\ SL1}$). Best top-1/top-5 accuracy between CRD and mAKD is marked with bold font.}
    \label{tab:crd_comparison}
\end{table*}

\textbf{ImageNet:} We used the same setup as in \cite{tian2019contrastive}. Since it is costly to perform a search for optimal $r_{GN}$ for ImageNet dataset, an uninformative prior\footnote{Discussed in section \ref{sec:discussion}.} $r_{GN}=1$ is used. The results are in table \ref{tab:imnet_exp}. While the CRD loss has better top-1 error, the mAKD loss achieves better top-5 error.
% For a further validation of mAKD loss, we performed experiments on ImageNet. 

\begin{table}
    \centering
    \input{figures/tables/imNet_exp.tex}
    \caption{Test error for training using mAKD on the ImageNet dataset. $r_{GN} = 1$ and mAKD($\tt{CS\ L2\ SL1}$) were used. The CRD results are from \cite{tian2019contrastive}.}
    \label{tab:imnet_exp}
\end{table}

\subsection{Ablation study for the importance of GNoRP}
\label{sec:dynamicBetaAblation}
To verify the effect of the GradNorm ratio preservation, in this study we examined different values of static $\lambda$ during the training. For each T-S pair the best performing $\lambda$ is found in a random search (40 runs per T-S pair, resulting in 520 runs in total)\footnote{Results of the random search are in supplementary material.}. Then the model is trained using the entire training set for five different random seeds\footnote{The same set of seeds as for CIFAR100 experiments are used.}. The results are in figure \ref{fig:beta_ablation}. We can see that the selected static $\lambda$, reported to the right of the plot, have a large variance across different T-S pairs, while the performance for the GNoRP with $r_{GN}=3.5$ (orange) is comparable, and often even better than the results with static $\lambda$ (blue). 

\begin{figure}
    \includegraphics[width=\linewidth]{figures/plots/optimal_beta_comparison}
    \caption{
    Performance with the static $\lambda$ (blue) and GradNorm ratio preservation (orange) on CIFAR100, using mAKD($\tt{CS\ L2\ SL1}$). 
    The average test accuracy plotted with min and max accuracy on the error bar. 
    The static $\lambda$ values are to the right of the plot.
    }
    \label{fig:beta_ablation}
\end{figure}

\subsection{Implementation details}
For all experiments we use hyper-parameters and teacher-student pairs as studied in \cite{tian2019contrastive}. For the experiments with \textbf{CIFAR100} dataset \cite{krizhevsky2009learning} all teacher-student pairs can be seen in table \ref{tab:crd_comparison}. Batch size is set to 64 and weight decay to 0.0005. SGD with momentum of 0.9 and learning rate of 0.05 is used for all cases except for ShuffleNet \cite{zhang2018shufflenet} and MobileNet \cite{howard2017mobilenets} architectures, where learning rate of 0.01 is applied. The experiments were run for 240 epochs and the learning rate was dropped by factor of 10 at epoch 150, 180 and 210. For the faster search experiments (sections \ref{subsec:combinatorialsearchresults}, \ref{sec:alphasearch}, and random search in section \ref{sec:dynamicBetaAblation}), we chose to run those with decreased number of epochs. Those experiments are run for 80 epochs while learning rate is dropped at epoch 50, 60 and 70.

For the \textbf{ImageNet} \cite{deng2009imagenet} experiments we used a pretrained resnet34 \cite{he2016deep} as teacher and resnet18 as student model. Batch size is set to 256, initial learning rate to 0.1, weight decay to 1e-4 and momentum to 0.9. We train for 100 epochs and learning rate is dropped by factor of 10 at epoch 30, 60 and 90.

In all search experiments \textbf{validation data} was used for evaluation which was created by randomly sampling 40\% of the training data.

To avoid unexpected influence from \textbf{GNoRP} we employ:
a separate optimiser for GNoRP (we use Adam with its default parameters in pyTorch), and
$\breve{\lambda} = \log(\lambda)$ as the variable for optimisation, to avoid negative values of $\lambda$. That is, we use $\lambda=\exp(\breve{\lambda})$ as the weighting parameter.
%\begin{itemize}
%    \item a separate optimiser for GNoRP, we use Adam with its default parameters in pyTorch. 
%    \item $\breve{\lambda} = \log(\lambda)$ as the variable for optimisation, to avoid negative values of $\lambda$. That is, we use $\lambda=\exp(\breve{\lambda})$ as the weighting parameter.
%\end{itemize}

For the evaluation of the mAKD loss in the \textbf{combinatorial search} (section \ref{subsec:combinatorialsearchresults}), we trained a linear classifier using a LinearSVC from scikit-learn \cite{scikit-learn}. All parameters of LinearSVC, except for dual, were kept as default. The dual was set to False in accordance with the recommendations in the documentation. Note that the GNoRP was not used in combinatorial search experiments.

